Matrix Inference in Growing Rank Regimes

The inference of a large symmetric signal-matrix $\mathbf{S} \in \mathbb{R}^{N\times N}$ corrupted by additive Gaussian noise, is considered for two regimes of growth of the rank $M$ as a function of $N$. For sub-linear ranks $M=\Theta(N^\alpha)$ with $\alpha\in(0,1)$ the mutual information and minimum mean-square error (MMSE) are derived for two classes of signal-matrices: (a) $\mathbf{S}=\mathbf{X}\mathbf{X}^\intercal$ with entries of $\mathbf{X}\in\mathbb{R}^{N\times M}$ independent identically distributed; (b) $\mathbf{S}$ sampled from a rotationally invariant distribution. Surprisingly, the formulas match the rank-one case. Two efficient algorithms are explored and conjectured to saturate the MMSE when no statistical-to-computational gap is present: (1) Decimation Approximate Message Passing; (2) a spectral algorithm based on a Rotation Invariant Estimator. For linear ranks $M=\Theta(N)$ the mutual information is rigorously derived for signal-matrices from a rotationally invariant distribution. Close connections with scalar inference in free probability are uncovered, which allow to deduce a simple formula for the MMSE as an integral involving the limiting spectral measure of the data matrix only. An interesting issue is whether the known information theoretic phase transitions for rank-one, and hence also sub-linear-rank, still persist in linear-rank. Our analysis suggests that only a smoothed-out trace of the transitions persists. Furthermore, the change of behavior between low and truly high-rank regimes only happens at the linear scale $\alpha=1$.

==> Main-paper/Figures/Rademacher/blank.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}[scale=0.25]

\end{tikzpicture}


==> Main-paper/Method.tex <==
\section{Methodology}

% This work combines four main tools, namely {\it spherical integrals}, {\it free probability}, the {\it replica method}, and {\it RIE's}. The use of the later has been sketched in the previous sections so we restrict the discussion to the first three.
% The {\it spherical integrals} involved in this work are defined 
% for two real symmetric matrices $\bA, \bB \in \bR^{N \times N}$ as
% $
%     \mathcal{I}_N(\bA, \bB) := \int D \bU \exp {\frac{N}{2} \Tr \bA \bU  \bB \bU^\intercal }
% $,
% where $D \bU$ is the Haar measure over the group of orthogonal matricesc The asymptotic behavior of HCIZ integrals in the symmetric case has been extensively studied in the literature, both in mathematics \cite{guionnet2002large} and in physics communities \cite{matytsin1994large}. In particular, it is possible to compute perturbative expansions, used in the matrix denoising problem in \cite{barbier2021statistical}, or sometimes work out explicit solutions to Matytsin's theory \cite{maillard2021perturbative}.

Besides spherical integrals, we also use results from \textit{free probability}. Free probability (see \cite{nica2006lectures, mingo2017free}) was initially introduced to study operator algebras, but has gained considerable importance in other realms due to its connection with the asymptotic behavior of random matrices. While free probability has been exploited in linear estimation and wireless communication problems \cite{muller2004random, verdu2010mismatched, nica2008free, reeves2018mutual}, the connection with matrix inference setting studied here is to the best of our knowledge new. The {\it replica method} \cite{mezard2009information} has been broadly used in inference and is known to lead to successful and provable --by other methods-- results for low rank problems. As already said for the linear rank regime, it still needs to be understood how to correctly use the method, if this is at all possible. Here we propose a new replica calculation for the large but sub-linear rank regime. As already mentioned, our prediction is compatible with existing rigorous results \cite{husson2022spherical}.


Among our various results, the proof of Theorem~\ref{statementMI} is particularly insightful due to the connections it establishes between matrix inference and free probability. To compute the integral over the MMSE \eqref{I-MMSE-rel}, first we show that the MMSE can be expressed as the free Fisher information of a non-commutative random variable, and then carry out the integration using basic relations in free probability to obtain the expression for the mutual information.
Let $X$ be a self-adjoint \textit{non-commutative} random variable $X$ associated to a probability measure  $\mu_X$ with compact support on the real line. According to \cite{voiculescu1993analogues, voiculescu1994analogues} the \textit{free entropy} $\chi(X)$ and the \textit{free Fisher information} $\Phi(X)$  are given as
\begin{align}
    \chi(X) &= \iint \ln |s-t| \mu_X(s) \mu_X(t) \, ds \,  dt + \frac{3}{4} + \frac{1}{2} \ln 2 \pi,
    \label{Free Entropy}\\
%
    \Phi(X) &= \frac{4 \pi^2}{3} \int \mu_X^3(s) \, ds.
    \label{Free Fisher}
\end{align}
Moreover, these two quantities are related through the relation:
\begin{equation}
    \chi(X) = \frac{1}{2} \int_0^{\infty} \Big( \frac{1}{1+t} - \Phi( X + \sqrt{t}Z ) \Big) \, dt + \frac{1}{2} \ln 2\pi + \frac{1}{2}
    \label{entropy-fisher}
\end{equation}
where $Z$ is a semicircular non-commutative random variable, and $X$ and $Z$ are {\it free}. We apply these relations to $X =S$ and $Z$, two free non-commutative random variables (not to confused with the $N\times N$ matrices $\bS$ and $\bZ$) associated to the probability measures $\rho_S$ and $\rho_{\rm sc}$. Since $S$ and $Z$ are free, the sum $\sqrt\gamma S + Z$ is a non-commutative random variable associated to the measure $\rho_{\sqrt\gamma S} \boxplus \rho_{\rm sc} = \rho_Y$. 
Clearly then
\eqref{asymp-MMSE-th} can be written in the free probability language as
\begin{equation}
    {\rm MMSE}(\gamma) = \frac{1}{\gamma} \Big( 1 - \Phi(\sqrt{\gamma}S + Z) \Big).
    \label{MMSE-freeFisher}
\end{equation}
Integrating both sides of \eqref{MMSE-freeFisher} over $\gamma$ and using \eqref{entropy-fisher} and \eqref{I-MMSE-rel} (the latter for $N\to \infty$), we conclude that (see details in Sec. 4 of SI)
\begin{equation}
  \frac{I_N(\bS;\bY)}{N^2}  \xrightarrow{N\to\infty} \frac{1}{2} \chi(\sqrt{\gamma} S + Z) - \frac{1}{4} \ln 2 \pi - \frac{1}{4}.
\end{equation}
This implies an explicit expression for the asymptotic mutual information. It is shown in \cite{voiculescu1997derivative} that $\Phi(\sqrt\gamma S + Z)$ is a continuous function of $\gamma$. Thus, \eqref{MMSE-freeFisher} implies that the ${\rm MMSE}(\gamma)$ is a continuous function of $\gamma$.

% \subsection*{Brief sketch of proof of Theorem 1}
% We explain here the main ideas of the proof of Theorem \ref{main-th}. Full details are found in \textcolor{blue}{SI}. We start from the posterior distribution of the model \eqref{observ-model}, which reads (up to some constants):
% \begin{equation}
%     \begin{split}
%         P_N (\bX | \bY) &\propto e^{-\frac{N}{4} \| \bY - \sqrt{\gamma}\bX \|_F^2 } P_{S,N}(\bX) \\
%         & \propto e^{\frac{N}{2} \Tr \big[ \sqrt{\gamma}\bX \bY - \frac{\gamma}{2} \bX^2 \big] } P_{S,N}(\bX)
%     \end{split}
%     \label{post-model1}
% \end{equation}
% The \textit{partition function} is defined as the normalizing factor of the posterior distribution \eqref{post-model1}:
% \begin{equation}
%     Z(\bY) = \int d \bX e^{\frac{N}{2} \Tr \big[ \sqrt{\gamma}\bX \bY - \frac{\gamma}{2} \bX^2 \big] } P_{S,N}(\bX)
%     \label{partition-function-def}
% \end{equation}
% and free energy is defined as:
% \begin{equation}
%     F_N (\gamma) = -\frac{1}{N^2} \bE_{Y} \big[ \ln Z(\bY) \big]
%     \label{free-energy-def}
% \end{equation}
% One can easily see that the free energy is linked to the (average) mutual information via the relation:
% \begin{equation*}
%     \frac{1}{N^2} \mathcal{I}_N(\bS;\bY) = F_N (\gamma) + \frac{\gamma}{4 N} \bE \big[ \Tr \bS^2 \big]
% \end{equation*}
% in which $\frac{1}{N} \bE \big[ \Tr \bS^2 \big]$ converges to the second moment of $\rho_S$ by assumption. Therefore, to prove theorem \ref{main-th}, it is enough to show that
% \begin{equation}
%      \lim_{N \to \infty} F_N (\gamma)  = \frac{\gamma}{4} \int x^2 \rho_{S}(x) \, dx - J[\rho_{\sqrt{\gamma}S}, \,\rho_{\sqrt{\gamma}S} \boxplus \rho_{\rm sc}]
%      \label{asymp-free energy}
% \end{equation}

% % To prove the asymptotic limit for the free energy $F_N(\gamma)$
% To prove the asymptotic limit in \eqref{asymp-free energy}, first, we show that this limit also holds for the free energy of a simpler model. Then, using the \textit{pseudo-Lipschitz} continuity of the free energy w.r.t. to a distance between two models which converges to $0$ as $N \to \infty$, we deduce that the same limit holds for the free energy of the original model.

%\showmatmethods{} 

